Moving target inference with hierarchical Bayesian models in synthetic aperture radar imagery

In synthetic aperture radar (SAR), images are formed by focusing the response of stationary objects to a single spatial location. On the other hand, moving targets cause phase errors in the standard formation of SAR images that cause displacement and defocusing effects. SAR imagery also contains significant sources of non-stationary spatially-varying noises, including antenna gain discrepancies, angular scintillation (glints) and complex speckle. In order to account for this intricate phenomenology, this work combines the knowledge of the physical, kinematic, and statistical properties of SAR imaging into a single unified Bayesian structure that simultaneously (a) estimates the nuisance parameters such as clutter distributions and antenna miscalibrations and (b) estimates the target signature required for detection/inference of the target state. Moreover, we provide a Monte Carlo estimate of the posterior distribution for the target state and nuisance parameters that infers the parameters of the model directly from the data, largely eliminating tuning of algorithm parameters. We demonstrate that our algorithm competes at least as well on a synthetic dataset as state-of-the-art algorithms for estimating sparse signals. Finally, performance analysis on a measured dataset demonstrates that the proposed algorithm is robust at detecting/estimating targets over a wide area and performs at least as well as popular algorithms for SAR moving target detection.

==> comparisons-magnitude.tex <==

\setlength{\unitlength}{0.85\textwidth}%


\def\xlabelxpos{-.065}
\def\xlabelypos{0.28}	% Change this to center x-axis label

\def\xtickypos{0.73}
\def\ytickxpos{-0.0675}

\def\ylabelxpos{-0.15}	% Change this to center y-axis label
\def\ylabelypos{0.8238}

% Note that the picture(x,y) sets the (x,y) size of the environment.
%   In order to make sure this isnt too much white space, set y to
%   be just a little bit bigger (~0.15) than the highest y-value used
%   in put(x0,y0).
\begin{picture}(1,0.80)%
    %\put(0,0){\includegraphics[width=\unitlength]{comparisons_small_scene_mag_cropped}}%
\put(0,0){\includegraphics[width=\unitlength]{comparisons_small_scene_mag_cropped}}%
    \put(-.015,0.78){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.2\unitlength}\centering $|\mathrm{Original}|$\end{minipage}}}%
    \put(0.2,0.785){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.2\unitlength}\centering $|\hat{{\bm M}}_{f,i}|$\end{minipage}}}%
    \put(0.405,.785){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.2\unitlength}\centering $\hat{\Pr}({\bm \Delta}_{f,i})$\end{minipage}}}%
    \put(0.605,.7775){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.2\unitlength}\centering DPCA (15 dB)\end{minipage}}}%
    \put(0.8,0.7775){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.2\unitlength}\centering DPCA (30 dB)\end{minipage}}}%
        \put(\ytickxpos,0.625){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.09134396\unitlength}\centering (a)\end{minipage}}}%
    \put(\ytickxpos,0.45){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.09134396\unitlength}\centering (b)\end{minipage}}}%
    \put(\ytickxpos,0.27){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.09134396\unitlength}\centering (c)\end{minipage}}}%
    \put(\ytickxpos,0.1){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.09134396\unitlength}\centering (d)\end{minipage}}}%
        \put(\xlabelxpos,0.37){\color[rgb]{0,0,0}\rotatebox{90}{\makebox(0,0)[lb]{\begin{minipage}{0.31\unitlength}\centering Scene 1\end{minipage}}}}%
    \put(\xlabelxpos,0.01){\color[rgb]{0,0,0}\rotatebox{90}{\makebox(0,0)[lb]{\begin{minipage}{0.31\unitlength}\centering Scene 2\end{minipage}}}}%
    \put(-0.0475,0.01){\line(0,1){0.32}}
    \put(-0.0475,0.37){\line(0,1){0.32}}

\end{picture}%




==> sar_Cramer.tex <==
\arrayrulecolor{defaultlinecolor}
\doublerulesepcolor{defaultlinecolor}

\subsection{Model}
Assume we have phase history measurements for $k$ antennas at each of $l$ frequencies and $m$ slow-time pulses.  Note that a SAR image is formed with a non-linear mapping of the phase-history to the imaging domain.  Range-Doppler images can be formed using a 2-dimensional FFT of the phase-history data, while other algorithms such as backprojection or polar format algorithm transform the phase-history data to the spatial $(x,y)$ domain.

Previous bounds for estimation error by Fasih \cite{fasih2010analysis} in SAR images have considered IID noise over all pulses, frequencies, and antennas.  In this section, we consider correlated noise across antennas as given in our SAR image model.  In particular, for the $l$-th frequency and $m$-th pulse, let us assume we have phase history measurements:
\begin{equation}
\glm = \mu_{lm}^k
+\varepsilon_{lm}^k,\quad k=1,\dots,K
\end{equation}
for 
\begin{align}
\mu_{lm}^k &= G\exp\set{j\left(\psi_{lm}^k+x(m\tau)h_{lm}^x+y(m\tau)h_{lm}^y\right)}\\
\psi_{lm}^k &= \psi_0 + (k-1)\phi,\\
x(m\tau) &= x_0 + (m\tau)v_x,\\
y(m\tau) &= y_0 + (m\tau)v_y,
\end{align}
where $\tau$ is the time between slow-time pulses and $\varepsilon_{lm}^k$ is zero-mean complex-valued additive noise with circular normal distribution:
\begin{equation}
\set{\varepsilon_{lm}^k}_{k=1}^K \sim \mathcal{CN}\left(0,\Lambda_{lm}\right).
\end{equation}
Note that $\varepsilon_{lm}^k$ is representative of the background variation that can possibly include clutter.  In particular, we assume that the covariance matrix is given by
\begin{equation}
\Lambda_{lm} = \lambda_{lm}^2\eyeKK + \kappa_{lm}^2 \oneK\oneK^T .
\end{equation}
where $\eyeKK$ is the $K\times K$ identity matrix and $\oneK$ is the all-ones vector of length $K$.  In the no-clutter case, we have $\lambda_{lm}^2=\sigma_v^2$ and $\kappa_{lm}^2=0$.  In the clutter-case, we have
\begin{align}
\lambda_{lm}^2 &= \sigma_v^2 + (\sigma_{lm}^s)^2 + (\sigma_{lm}^x)^2 + \delta^{y,m}(\sigma_{lm}^y)^2\\
\kappa_{lm}^2 &= \rho_{lm}^s(\sigma_{lm}^s)^2 + \rho_{lm}^x(\sigma_{lm}^x)^2 + \delta^{y,m}\rho_{lm}^y(\sigma_{lm}^y)^2
\end{align}
Let the parameter vector be defined as 
\begin{equation}
\Theta = \set{x_0,y_0,v_x,v_y,G,\psi_0,\phi}
\end{equation}
Then the Fisher information matrix is given by the elemnent-wise definition by Kay \cite{Kay-98-detec-theo}:
\begin{equation}
[\mathrm{FIM}]_{uv} = 2\sum\limits_{l,m}\Re\set{\left(\frac{\partial\vec{u}_{lm}}{\partial\theta_u}\right)^H\Lambda_{lm}^{-1}\left(\frac{\partial\vec{u}_{lm}}{\partial\theta_v}\right)} +\sum\limits_{l,m}\mathrm{trace}\left(\Lambda_{lm}^{-1}\frac{\partial\Lambda_{lm}}{\partial\theta_u}\Lambda_{lm}^{-1}\frac{\partial\Lambda_{lm}}{\partial\theta_v}\right)
\end{equation}
where $\mu_{lm} = \set{\mu_{lm}^k}_{k=1}^K$.

\subsection{Mean term}
Let us first focus on the FIM contribution from the mean component:
\begin{equation}
\label{sar-eq:FIM-mean}
2\sum\limits_{l,m}\Re\set{\left(\frac{\partial\vec{\mu}_{lm}}{\partial\theta_u}\right)^H\Lambda_{lm}^{-1}\left(\frac{\partial\vec{\mu}_{lm}}{\partial\theta_v}\right)}
\end{equation}
The following table gives the partial derivatives for each parameter in $\Theta$ for 
\begin{equation}
\alpha_{lm} = \exp\set{j\left(\psi_0+x(m\tau)h_{lm}^x+y(m\tau)h_{lm}^y\right)}
\end{equation}
%\renewcommand{\arraystretch}{1.5}

\begin{table}[thp]
\caption{Partial derivatives for FIM derivation}
\label{sar-table:FIM-partial-derivatives}
\centering
\begin{tabular}{|l|c|c|}
\hline
Parameter, $\theta_u$ & $\frac{\partial\mu_{lm}^k}{\partial\theta_u}$ & $u_k \trieq\frac{\partial\mu_{lm}^k}{\partial\theta_u}/(\alpha_{lm}e^{j\phi(k-1)})$\\
\hline\hline
$x_0$ & {$Gh_{lm}^x\alpha_{lm}  e^{j\phi(k-1)} $} & {$Gh_{lm}^x$}\\\hline
$y_0$ & {$Gh_{lm}^y\alpha_{lm}  e^{j\phi(k-1)} $} & {$Gh_{lm}^y$}\\\hline
$v_x$ & {$Gm\tau h_{lm}^x\alpha_{lm}  e^{j\phi(k-1)} $} & {$Gm\tau h_{lm}^x$}\\\hline
$v_y$ & {$Gm\tau h_{lm}^y\alpha_{lm}  e^{j\phi(k-1)} $} & {$Gm\tau h_{lm}^y$}\\\hline
$G$ & {$\alpha_{lm}  e^{j\phi(k-1)} $} &1\\\hline
$\psi_0$ & {$G\alpha_{lm}  e^{j\phi(k-1)} $} &$G$\\\hline
$\phi$ & {$G\alpha_{lm}(k-1)e^{j\phi(k-1)} $} &{$G(k-1)$}\\\hline
\end{tabular}
\end{table}
Note that the last column of Table \ref{sar-table:FIM-partial-derivatives} shows that all components at the $k$-antenna share the same dependence on the parameter $\alpha_{lm}$ and a phase component $e^{j\phi(k-1)}$.  Define the vectors
\begin{equation}
\vec{u}=
\left[\begin{array}{*{20}c}
u_1\\u_2e^{j\phi}\\\vdots\\u_Ke^{j\phi(K-1)}
\end{array}\right],
\vec{v}=
\left[\begin{array}{*{20}c}
v_1\\v_2e^{j\phi}\\\vdots\\v_Ke^{j\phi(K-1)}
\end{array}\right]
\end{equation}
where $u_k$ and $v_k$ are given by the third column in Table \ref{sar-table:FIM-partial-derivatives} for partial derivatives with respect to $\theta_u$ and $\theta_v$ respectively.  Then the summand in equation (\ref{sar-eq:FIM-mean}) can be written as
\begin{equation}
\label{sar-eq:FIM-mean-summand}
\begin{split}
\Re\set{\left(\frac{\partial\vec{\mu}_{lm}}{\partial\theta_u}\right)^H\Lambda_{lm}^{-1}\left(\frac{\partial\vec{\mu}_{lm}}{\partial\theta_v}\right)} &=\Re\set{\left(\alpha_{lm}\vec{u}\right)^H \Lambda_{lm}^{-1} \left(\alpha_{lm}\vec{v}\right)}\\
&=\Re\set{ \alpha_{lm}^*\alpha_{lm} \vec{u}^H\Lambda_{lm}^{-1} \vec{v}}\\
&=\Re\set{ \vec{u}^H\Lambda_{lm}^{-1} \vec{v}}
\end{split}
\end{equation}
where we note that $\alpha_{lm}^*\alpha_{lm}=1$.  Note that $u$ and $v$ do not depend on the target state $(x_0,y_0,v_x,v_y)$.  Thus, the mean contribution to the FIM will be independent of the target state.  Furthermore, if $\Lambda_{lm}$ does not depend on these parameters as in the clutter-free case, then the FIM and CRB will be independent of the target parameters; i.e., we should be able to find an algorithm that can track the target equally well regardless of its actual state.

To simplify the computation of the mean contribution to the FIM, consider the fact that
\begin{align}
\Lambda_{lm}^{-1} &= \left[\kappa_{lm}^2\oneK\oneK^T + \lambda_{lm}^2\eyeKK\right]^{-1}\\
&= \lambda_{lm}^{-2}\left(\eyeKK-\frac{\kappa_{lm}^2}{K\kappa_{lm}^2+\lambda_{lm}^2}\oneK\oneK^T\right)\\
&= L_{lm}^0 \eyeKK + L_{lm}^1 \oneK\oneK^T,
\end{align}
where
\begin{align}
L_{lm}^0 &=  \lambda_{lm}^{-2},\\
L_{lm}^1 &=  \frac{\kappa_{lm}^2}{K\kappa_{lm}^2\lambda_{lm}^2+\lambda_{lm}^4}.
\end{align}
Then equation (\ref{sar-eq:FIM-mean-summand}) becomes
\begin{equation}
\begin{split}
\Re\set{ \vec{u}^H\Lambda_{lm}^{-1} \vec{v} }&= \Re\set{ \vec{u}^H \left(L_{lm}^0 \eyeKK + L_{lm}^1 \oneK\oneK^T\right) \vec{v} }\\
&= L_{lm}^0 \sum_k u_kv_k + L_{lm}^1\Re\set{\left(\sum_{k} u_ke^{-j\phi(k-1)}\right)\left(\sum_{k} v_ke^{j\phi(k-1)}\right)}\\
&= L_{lm}^0 \sum_k u_kv_k + L_{lm}^1\Re\set{\left(\sum_{k}\sum_{n} u_kv_ne^{j\phi(n-1-k+1)}\right)}\\
&= L_{lm}^0 \sum_k u_kv_k + L_{lm}^1\sum_{k}\sum_{n} u_kv_n\Re\set{e^{j\phi(n-k)}}\\
&= L_{lm}^0 \sum_k u_kv_k + L_{lm}^1\sum_{k}\sum_{n} u_kv_n\cos(\phi(n-k))
\end{split}
\end{equation}
This equation simplies further when $u_k=u$ or $v_k=v$ as is the case for all parameters except $\phi$.  In particular, if $u_k=u$ and $v_k=v$, then:
\begin{equation}
\begin{split}
\Re\set{ \vec{u}^H\Lambda_{lm}^{-1} \vec{v} }&= (uv)\left(K L_{lm}^0 + L_{lm}^1\sum_{k}\sum_{n} \cos(\phi(n-k)) \right)\\
&= (uv)\left(K L_{lm}^0 + \alpha_\phi L_{lm}^1 \right),
\end{split}
\end{equation}
where $\alpha_\phi = \sum_{k,n} \cos(\phi(n-k))$.  In the case where $\theta_u\neq\phi$ and $\theta_v=\phi$, we have
\begin{equation}
\begin{split}
\Re\set{ \vec{u}^H\Lambda_{lm}^{-1} \vec{v} }&= L_{lm}^0\left(Gu\sum_k(k-1)\right) +  L_{lm}^1\left(Gu\sum_k\sum_n (n-1)\cos(\phi(n-k))\right)\\
&= Gu\left(L_{lm}^0\frac{K(K-1)}{2}+ L_{lm}^1\sum_k\sum_n (n-1)\cos(\phi(n-k))\right)\\
&= Gu\left(L_{lm}^0\frac{K(K-1)}{2}+ L_{lm}^1(\alpha_\phi^n-\alpha_\phi)\right),
\end{split}
\end{equation}
where
\begin{equation}
\alpha_\phi^n = \sum_k\sum_n n\cos(\phi(n-k))
\end{equation}
Finally, in the case where $\theta_u=\theta_v=\phi$, we have
\begin{equation}
\begin{split}
\Re\set{ \vec{u}^H\Lambda_{lm}^{-1} \vec{v} }&= L_{lm}^0\left(G^2\sum_k(k-1)^2\right) \\
&+  L_{lm}^1\left(G^2\sum_k\sum_n (k-1)(n-1)\cos(\phi(n-k))\right)\\
&= G^2\left(L_{lm}^0\frac{K(K-1)(2K-1)}{6}+ L_{lm}^1(\alpha_\phi^{kn}-2\alpha_\phi^{n}+\alpha_\phi)\right),\\
\end{split}
\end{equation}
where
\begin{equation}
\alpha_\phi^{kn} = \sum_k\sum_n kn\cos(\phi(n-k))
\end{equation}
In all cases, the summand can be represented as
\begin{equation}
\Re\set{ \vec{u}^H\Lambda_{lm}^{-1} \vec{v} } = \beta_{uv}^0 L_{lm}^0 + \beta_{uv}^0 L_{lm}^1,
\end{equation}
where the parameters $\beta_{uv}^0,\beta_{uv}^1$ are given in Table \ref{sar-table:FIM-mean-beta}.

\begin{table}[thp]
\caption{$\beta_{uv}^0,\beta_{uv}^1$ parameters}
\label{sar-table:FIM-mean-beta}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
$\theta_u \in$ & $\theta_v \in$ & $\beta_{uv}^0$ & $\beta_{uv}^1$\\
\hline\hline
$\set{\begin{array}{cc}
x_0,y_0,v_x,\\
v_y,G,\psi_0
\end{array}
}$ & $\set{\begin{array}{cc}
x_0,y_0,v_x,\\
v_y,G,\psi_0
\end{array}
}$ & $uvK$ & $uv\alpha_\phi$\\
\hline
$\set{\begin{array}{cc}
x_0,y_0,v_x,\\
v_y,G,\psi_0
\end{array}
}$ & $\set{\phi}$ & $\frac{GuK(K-1)}{2}$ & $Gu(\alpha_\phi^n-\alpha_\phi)$\\
\hline
 $\set{\phi}$ & $\set{\begin{array}{cc}
x_0,y_0,v_x,\\
v_y,G,\psi_0
\end{array}
}$ &$\frac{GvK(K-1)}{2}$ & $Gv(\alpha_\phi^n-\alpha_\phi)$\\
\hline
 $\set{\phi}$ & $\set{\phi}$ &$\frac{G^2K(K-1)(2K-1)}{6}$ & $G^2(\alpha_\phi^{kn}-2\alpha_\phi^n+\alpha_\phi)$\\
\hline \end{tabular}
\end{table}

\subsection{Covariance term}
We now consider the FIM contribution from the covariance component:
\begin{equation}
\mathrm{trace}\left(\Lambda_{lm}^{-1}\frac{\partial\Lambda_{lm}}{\partial\theta_u}\Lambda_{lm}^{-1}\frac{\partial\Lambda_{lm}}{\partial\theta_v}\right)
\end{equation}
In general, it may difficult to determine the effect of the target state parameters on the noise covariance matrix.  In this section, we suppose that within the small regions where the target signature will appear over a CPI, we can approximate this dependence with a linear map from spatial coordinates to the parameters $\rho,\sigma^2$ of our covariance matrix.  In particular
\begin{equation}
\begin{split}
\kappa^2(x,y) &= \kappa_0^2 + x\gamma_x^\kappa + y\gamma_y^\kappa,\\
\lambda^2(x,y) &= \lambda_0^2 + x\gamma_x^\lambda + y\gamma_y^\lambda.
\end{split}
\end{equation}
for parameters $(\kappa_0^2,\lambda_0^2,\gamma_x^\kappa,\gamma_y^\kappa,\gamma_x^\lambda,\gamma_y^\lambda,)$ that can be fitted from our SAR image model.  In this case, we have
\begin{equation}
\begin{split}
\frac{\partial\Lambda_{lm}}{\partial\theta_u} &= \frac{\partial}{\partial\theta_u}\left\{\kappa_{lm}^2 \eyeKK + \lambda_{lm}^2 \oneK\oneK^T\right\}\\
& = \frac{\partial\kappa_{lm}^2}{\partial\theta_u} \eyeKK + \frac{\partial\lambda_{lm}^2}{\partial\theta_u}\oneK\oneK^T ,
\end{split}
\end{equation}
For example, when $\theta_u=x_0$, we have
\begin{equation}
 \frac{\partial\kappa_{lm}^2}{\partial x_0}=\gamma_x^\kappa,\  \frac{\partial\lambda_{lm}^2}{\partial x_0}=\gamma_x^\lambda.
\end{equation}
Then we have
\begin{equation}
\begin{split}
\Lambda_{lm}^{-1}\frac{\partial\Lambda_{lm}}{\partial\theta_u} &= \left( L_{lm}^0 \eyeKK + L_{lm}^1 \oneK\oneK^T\right)\left( \frac{\partial\kappa_{lm}^2}{\partial\theta_u} \eyeKK + \frac{\partial\lambda_{lm}^2}{\partial\theta_u}\oneK\oneK^T\right),\\
&= \tildeBetaEye{u} \eyeKK + \tildeBetaOneOne{u} \oneK\oneK^T,
\end{split}
\end{equation}
where
\begin{align}
\tildeBetaEye{u} &= L_{lm}^0\frac{\partial\kappa_{lm}^2}{\partial\theta_u},\\
\tildeBetaOneOne{u} &= L_{lm}^1\frac{\partial\kappa_{lm}^2}{\partial\theta_u} + \left(L_{lm}^0+ KL_{lm}^1\right)\frac{\partial\lambda_{lm}^2}{\partial\theta_u}.
\end{align}
Finally, we have
\begin{equation}
\begin{split}
\mathrm{trace}&\left(\Lambda_{lm}^{-1}\frac{\partial\Lambda_{lm}}{\partial\theta_u}\Lambda_{lm}^{-1}\frac{\partial\Lambda_{lm}}{\partial\theta_v}\right)
\\
&= \mathrm{trace}\set{\left(\tildeBetaEye{u} \eyeKK + \tildeBetaOneOne{u} \oneK\oneK^T\right)\left(\tildeBetaEye{v} \eyeKK + \tildeBetaOneOne{v} \oneK\oneK^T\right)}\\
&=\mathrm{trace}\set{\tildeBetaEye{u}\tildeBetaEye{v}\eyeKK + \left(\tildeBetaEye{u}\tildeBetaOneOne{v}+\tildeBetaEye{v}\tildeBetaOneOne{u}+K\tildeBetaOneOne{u}\tildeBetaOneOne{v}\right)\oneK\oneK^T} \\
&= K\left(\tildeBetaEye{u}\tildeBetaEye{v} + \tildeBetaEye{u}\tildeBetaOneOne{v}+\tildeBetaEye{v}\tildeBetaOneOne{u}+K\tildeBetaOneOne{u}\tildeBetaOneOne{v}\right)
\end{split}
\end{equation}
This equation may simplify in some cases, though we won't give all details here.  However, it should be noted that the original derivatives $\frac{\partial\sigma_{lm}^2}{\partial\theta_u}$ and $\frac{\partial\rho}{\partial\theta_u}$ are non-zero only for $\theta_u\in\set{x_0,y_0,v_x,v_y}$.  Moreover, if either $\theta_u$ or $\theta_v$ does not belong to this set, then our trace will equal zero.  Thus, we only have to compute this term for a subset of the elements of the FIM.

